Noisy Interpolation Learning with Shallow Univariate ReLU Networks

Understanding how overparameterized neural networks generalize despite perfect interpolation of noisy training data is a fundamental question. Mallinar et. al. 2022 noted that neural networks seem to often exhibit ``tempered overfitting'', wherein the population risk does not converge to the Bayes optimal error, but neither does it approach infinity, yielding non-trivial generalization. However, this has not been studied rigorously. We provide the first rigorous analysis of the overfitting behavior of regression with minimum norm ($\ell_2$ of weights), focusing on univariate two-layer ReLU networks. We show overfitting is tempered (with high probability) when measured with respect to the $L_1$ loss, but also show that the situation is more complex than suggested by Mallinar et. al., and overfitting is catastrophic with respect to the $L_2$ loss, or when taking an expectation over the training set.

==> ICLR2024/macros.tex <==
% General:

\newcommand{\Leq}[1]{\ensuremath{\underset{\textnormal{#1}}\leq}}
\newcommand{\Geq}[1]{\ensuremath{\underset{\textnormal{#1}}\geq}}
\newcommand{\Eq}[1]{\ensuremath{\underset{\textnormal{#1}}=}}


\newcommand{\tvd}[2]{\ensuremath{\norm{#1 - #2}_{\mathrm{tvd}}}}
\newcommand{\Ot}{\ensuremath{\widetilde{O}}}
\newcommand{\Paren}[1]{\Big(#1\Big)}
\newcommand{\Bracket}[1]{\Big[#1\Big]}
\newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\paren}[1]{\ensuremath{\left(#1\right)}\xspace}
\newcommand{\card}[1]{\left\vert{#1}\right\vert}
\newcommand{\Omgt}{\ensuremath{\widetilde{\Omega}}}
\newcommand{\half}{\ensuremath{{1 \over 2}}}

\newcommand{\IR}{\ensuremath{\mathbb{R}}}
\newcommand{\IQ}{\ensuremath{\mathbb{Q}}}
\newcommand{\IIZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\IN}{\ensuremath{\mathbb{N}}}
\newcommand{\IS}{\ensuremath{\mathbb{S}}}
\newcommand{\IB}{\ensuremath{\mathbb{B}}}



\newcommand{\lee}{\leqslant}
\newcommand{\gee}{\geqslant}
\newcommand{\prob}[1]{\Pr\paren{#1}}
\newcommand{\expect}[1]{\Exp\bracket{#1}}
\newcommand{\var}[1]{\textnormal{Var}\bracket{#1}}
\newcommand{\cov}[1]{\textnormal{Cov}\bracket{#1}}
\newcommand{\eexp}[1]{\exp\paren{#1}}
\newcommand{\set}[1]{\ensuremath{\left\{ #1 \right\}}}
\newcommand{\poly}{\mbox{\rm poly}}
\newcommand{\polylog}{\mbox{\rm  polylog}}

\newcommand{\OPT}{\ensuremath{\mbox{\sc opt}}\xspace}
\newcommand{\opt}{\textnormal{\ensuremath{\mbox{opt}}}\xspace}
\newcommand{\APX}{\ensuremath{\mbox{APX}}}
\newcommand{\apx}{\ensuremath{\mbox{apx}}}
\newcommand{\ALG}{\ensuremath{\mbox{\sc alg}}\xspace}
\newcommand{\alg}{\ensuremath{\mathcal{A}}\xspace}

\DeclareMathOperator*{\Exp}{\ensuremath{{\mathbb{E}}}}
\DeclareMathOperator*{\Prob}{\ensuremath{\mathbb{P}}}
\renewcommand{\Pr}{\Prob}
\newcommand{\EX}{\Exp}
\newcommand{\Ex}{\Exp}
\newcommand{\bigO}[1]{\ensuremath{O\Paren{#1}}}

\newcommand{\etal}{{\it et al.\,}}
\newcommand{\goodetal}{{\it et al.\/}}


% Table: 
\newenvironment{tbox}{\begin{tcolorbox}[
		enlarge top by=5pt,
		enlarge bottom by=5pt,
		 breakable,
		 boxsep=0pt,
                  left=4pt,
                  right=4pt,
                  top=10pt,
                  arc=0pt,
                  boxrule=1pt,toprule=1pt,
                  colback=white
                  ]%%
	}
{\end{tcolorbox}}

\newcommand{\textbox}[2]{
{
\begin{tbox}
\textbf{#1}
{#2}
\end{tbox}
}
}

% Probabilistic notation:  
\newcommand{\event}{\ensuremath{\mathcal{E}}}

\newcommand{\rA}{\rv{A}}
\newcommand{\rB}{\rv{B}}
\newcommand{\rC}{\rv{C}}
\newcommand{\rD}{\rv{D}}
\newcommand{\rE}{\rv{E}}

\newcommand{\supp}[1]{\ensuremath{\textnormal{\text{supp}}(#1)}}
\newcommand{\distribution}[1]{\ensuremath{\textnormal{dist}(#1)}\xspace}
\newcommand{\distributions}[2]{\ensuremath{\textnormal{dist}_{#2}(#1)}\xspace}

\newcommand{\kl}[2]{\ensuremath{\mathbb{D}(#1~||~#2)}}
\newcommand{\II}{\ensuremath{\mathbb{I}}}
\newcommand{\HH}{\ensuremath{\mathbb{H}}}
\newcommand{\mi}[2]{\ensuremath{\def\mione{#1}\def\mitwo{#2}\mireal}}
\newcommand{\mireal}[1][]{
  \ifx\relax#1\relax%
    \II(\mione \,; \mitwo)%
  \else%
    \II(\mione \,; \mitwo\mid #1)%
  \fi
}
\newcommand{\en}[1]{\ensuremath{\HH(#1)}}

\newcommand{\itfacts}[1]{\Cref{fact:it-facts}-(\ref{part:#1})\xspace}

% Paper: 

\newcommand{\vareps}{\varepsilon}

\newcommand{\cD}{\mathcal{D}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bOne}{\mathbf{1}}
\newcommand{\odd}{B}
\newcommand{\even}{A}

% \newcommand{\Itvd}{I_{\mathrm{tvd}}}

\newcommand{\adv}{\mathrm{bias}}
\newcommand{\Pyes}{P^{\textnormal{\textsf{Yes}}}}
\newcommand{\Pno}{P^{\textnormal{\textsf{No}}}}
\newcommand{\Pdelta}{P_{\Delta}}


\newcommand{\mnote}[1]{ \marginpar{\tiny\bf
           \begin{minipage}[t]{0.5in}
             \raggedright \color{red}#1
          \end{minipage}}}


\newcommand{\block}[1]{\ensuremath{{B}^{#1}}}

\newcommand{\Sb}[1]{S^{#1}}
\newcommand{\Tb}[1]{T^{#1}}
\newcommand{\Ub}[1]{U^{#1}}
\newcommand{\Vb}[1]{V^{#1}}
\newcommand{\Eb}[1]{E^{#1}}
\newcommand{\Mb}[1]{M^{#1}}
\newcommand{\Pb}[1]{P^{#1}}
\newcommand{\Mc}{M^{con}}

\newcommand{\dist}{\ensuremath{\mathcal{D}}}
\newcommand{\bdist}{\overline{\dist}}

\newcommand{\PP}[1]{{P}^{#1}}
\newcommand{\Pstar}{P^*}
\newcommand{\PPstar}{{P^*}}

\newcommand{\prot}{\pi}
\newcommand{\Prot}{\Pi}
\newcommand{\ProtA}{\Prot_A}
\newcommand{\ProtB}{\Prot_B}




\newcommand{\BBo}{\mathbf{B}_{odd}}
\newcommand{\BBe}{\mathbf{B}_{even}}

\newcommand{\MM}{\ensuremath{{M}}}

\newcommand{\RR}{\ensuremath{\mathbf{R}}}

\renewcommand{\SS}{\ensuremath{\mathcal{S}}}

\newcommand{\finalmatching}{\ensuremath{\textnormal{\textbf{Final-Matching Testing}}}\xspace}

\newcommand{\FMT}{\ensuremath{\textnormal{\textbf{FMT}}}\xspace}
\newcommand{\fmt}{\ensuremath{\textnormal{FMT}}\xspace}


\newcommand{\Myes}{\ensuremath{P^{\textnormal{\textsf{Yes}}}}}
\newcommand{\Mno}{\ensuremath{P^{\textnormal{\textsf{No}}}}}
\newcommand{\Mdelta}{\ensuremath{P_{\Delta}}}
\newcommand{\distFMTyes}{\ensuremath{\dist^{\textnormal{\textsf{Yes}}}}}
\newcommand{\distFMTno}{\ensuremath{\dist^{\textnormal{\textsf{No}}}}}

\newcommand{\distFMT}{\ensuremath{\dist_{\textnormal{\textsf{FMT}}}}}
\newcommand{\PFMT}{\ensuremath{\dist_{P, \textnormal{\textsf{FMT}}}}}

\newcommand{\errs}{\ensuremath{\textnormal{errs}}}

%Symbols
\newcommand{\ip}[2]{\ensuremath{\langle  #1, #2 \rangle}}
\newcommand{\norm}[1]{\ensuremath{\left\lVert #1 \right\rVert}}
\newcommand{\A}[1]{\ensuremath{W^{(#1)}}}
\newcommand{\Em}[1]{\ensuremath{\mathcal{E}^{(#1)}}}
\newcommand{\um}[1]{\ensuremath{u^{(#1)}}}
\newcommand{\sm}[1]{\ensuremath{s^{(#1)}}}
\newcommand{\smallnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert}}
\newcommand{\infnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert}_{\infty}}
\newcommand{\twonorm}[1]{\ensuremath{\left\lVert #1 \right\rVert}_{2}}
\newcommand{\twotoinfnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert}_{2\rightarrow \infty}}
\newcommand{\rank}{\textnormal{{rank}}}
\newcommand{\edge}{e}
\newcommand{\hsparse}{\mathsf{HSparse}}
\newcommand{\hsbm}{\textnormal{HSBM}}
\newcommand{\her}{\mathsf{HER}}
\newcommand{\param}{\mathbb{\theta}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\lip}[1]{\norm{#1}_{\text{Lip}}}
\newcommand{\unif}{\text{Uniform}}
\newcommand{\ridgeless}{\text{RidgeLessReLU}}
\newcommand{\iid}{\stackrel{\mathrm{ i.i.d.}}{\sim}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\curv}{\mathsf{curv}}

%\newcommand{\dist}{\mathcal{D}}

\newcommand{\ifcomments}{\iftrue}
%\newcommand{\nirmit}[1]{{\ifcomments\color{orange} [\textbf{Nirmit:}  #1]}\fi}
%%%%%%%%%%%
%\newcommand{\gal}[1]{{\ifcomments\color{red} [\textbf{Gal:}  #1]}\fi}
%\newcommand{\nati}[1]{{\ifcomments\color{green} [\textbf{Nati:}  #1]}\fi}
\newcommand{\reals}{{\mathbb R}}
\newcommand{\nat}{{\mathbb N}}
\newcommand{\removed}[1]{}

%%%%%%%%%%%%
%algorithms
\usepackage{algorithm}
\usepackage{algpseudocode}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\makeatletter
\newenvironment{breakablealgorithm}
  {% \begin{breakablealgorithm}
   \begin{center}
     \refstepcounter{algorithm}% New algorithm
     \hrule height.8pt depth0pt \kern2pt% \@fs@pre for \@fs@ruled
     \renewcommand{\caption}[2][\relax]{% Make a new \caption
       {\raggedright\textbf{\ALG@name~\thealgorithm} ##2\par}%
       \ifx\relax##1\relax % #1 is \relax
         \addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##2}%
       \else % #1 is not \relax
         \addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##1}%
       \fi
       \kern2pt\hrule\kern2pt
     }
  }{% \end{breakablealgorithm}
     \kern2pt\hrule\relax% \@fs@post for \@fs@ruled
   \end{center}
  }
\makeatother

==> ICLR2024/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICLR2024/paper.tex <==
\section{Introduction}

A recent realization is that, although sometimes overfitting can be catastrophic as suggested by our classic learning theory understanding, in other cases overfitting may not be so catastrophic. In fact, even \textit{interpolation learning}, which entails achieving zero training error with noisy data, can still allow for good generalization, and even consistency \citep{zhang2017rethinkinggeneralization,belkin2018overfittingperfectfitting}.
This has led to efforts towards understanding the nature of overfitting: how \textit{benign} or \textit{catastrophic} it is, and what determines this behavior, in different settings and using different models. 

Although interest in benign overfitting stems from the empirical success of interpolating large neural networks, theoretical study so far has been mostly limited to linear and kernel methods, or to classification settings where the data is already linearly separable, with very high data dimension (tending to infinity as the sample size grows)\footnote{Minimum $\ell_2$ norm linear prediction (aka ridgeless regression) with noisy labels and (sub-)Gaussian features has been studied extensively 
\citep[e.g.][]{hastie2020surprises,belkin2020two,bartlett2020benignpnas,muthukumar2020harmless,negrea2020defense,chinot2020robustness,koehler2021uniform,wu2020optimal,tsigler2020benign,zhou2022non,wang2022tight,chatterji2021interplay,bartlett2021failures,shamir2022implicit,ghosh2022universal,chatterji2020linearnoise,wang2021binary,cao2021benign,muthukumar2021classification,montanari2020maxmarginasymptotics,liang2021interpolating,thrampoulidis2020theoretical,wang2021benignmulticlass,donhauser2022fastrates,frei2023benign}, and noisy minimum $\ell_1$ linear prediction (aka Basis Persuit) has also been considered \citep[e.g.][]{ju2020overfitting,koehler2021uniform,wang2022tight}.  Either way, these analyses are all in the high dimensional setting, with dimension going to infinity, since to allow for interpolation the dimension must be high, higher than the number of samples. Kernel methods amount to a minimum $\ell_2$ norm linear prediction, with very non-Gaussian features.  But existing analyses of interpolation learning with kernel methods rely on ``Gaussian Universality'': either assuming as an ansatz the behavior is as for Gaussian features \citep{mallinar2022benign} or establishing this rigorously in certain high dimensional scalings \citep{hastie2019surprises,misiakiewicz2022spectrum,mei2022generalization}.
In particular, such analyses are only valid when the input dimension goes to infinity (though possibly slower than the number of samples) and not for fixed low or moderate dimensions.
\citet{frei2022benign,frei2023benign,cao2022benign,kou2023benign} study interpolation learning with neural networks, but only with high input dimension and when the data is interpolatable also with a linear predictor---in these cases, although non-linear neural networks are used, the results show they behave similarly to linear predictors. 
\citet{manoj2023interpolation} take the other extreme and study interpolation learning with ``short programs'', which are certainly non-linear, but this is an abstract model that does not directly capture learning with neural networks.}. %Finally, we note that in a concurrent and independent work, \citet{kornowski2023tempered} studied interpolation learning in classification with univariate ReLU networks, as well as in certain high-dimensional settings.}. 
But what about noisy interpolation learning in low dimensions, using neural networks?

\citet{mallinar2022benign} conducted simulations with neural networks and observed  \textit{``tempered"} overfitting:  the asymptotic risk does not approach the Bayes-optimal risk (there is no consistency), but neither does it diverge to infinity catastrophically.  Such ``tempered'' behavior is well understood for $1$-nearest neighbor, where the asymptotic risk is roughly twice the Bayes risk \citep{cover1967nearest}, and \citeauthor{mallinar2022benign} heuristically explain it also for some kernel methods. However, we do not have a satisfying and rigorous understanding of such behavior in neural networks, nor a more quantitative understanding of just how bad the risk might be when interpolating noisy data using a neural net.

In this paper, we begin rigorously studying the effect of overfitting in the noisy regression setting, with neural networks in low dimensions, where the data is {\em not} linearly interpolatable. Specifically, we study interpolation learning of univariate data (i.e.~in one dimension) using a two-layer ReLU network (with a skip connection), which is a predictor $f_{\theta,a_0,b_0}:\IR \rightarrow \IR$ given by:
\begin{equation}\label{eq:net}
f_{\theta,a_0,b_0}(x) = \sum_{j=1}^m a_j (w_j x + b_j)_+ +  a_0 x + b_0~,
\end{equation}
where $\theta \in \reals^{3m}$ denotes the weights (parameters) $\{a_j,w_j,b_j\}_{j=1}^m$.  To allow for interpolation we do not limit the width $m$, and learn by minimizing the norm of the weights \citep{savarese2019infinite,ergen2021convex,hanin2021ridgeless,debarre2022sparsest,boursier2023penalising}:
\begin{equation} \label{eq:main_problem}
    \hat{f}_S = \arg\min_{f_{\theta,a_0,b_0}} \norm{\theta}^2 \;\text{ s.t. } \; \forall i \in [n],\; f_{\theta,a_0,b_0}(x_i)=y_i~\; \textrm{where $S=\{(x_1,y_1),\ldots,(x_n,y_n)\}$}.
\end{equation}

Following \citet{boursier2023penalising} we allow an unregularized skip-connection in \eqref{eq:net}, where the weights $a_0,b_0$ of this skip connection are not included in the norm $\norm{\theta}$ in \eqref{eq:main_problem}. This skip connection avoids some complications and allows better characterizing $\hat{f}_S$ but does not meaningfully change the behavior (see Section~\ref{sec:review_min_norm_nets}).

\paragraph{Why min norm?} Using unbounded size minimum weight-norm networks is natural for interpolation learning.  It parallels the study of minimum norm high (even infinite) dimension linear predictors.  For interpolation, we must allow the number of parameters to increase as the sample size increases.  But to have any hope of generalization, we must choose among the infinitely many zero training error networks somehow, and it seems that some sort of explicit or implicit low norm bias is the driving force in learning with large overparameterized neural networks \citep{neyshabur2014search}.  Seeking minimum $\ell_2$ norm weights is natural, e.g.~as a result of small weight decay. Even without explicit weight decay, optimizing using gradient descent is also related to an implicit bias toward low $\ell_2$ norm: this can be made precise for linear models and for classification with ReLU networks \citep{chizat2020implicit,safran2022effective}. For regression with ReLU networks, as we study here, 
the implicit bias is not well understood (see \cite{vardi2023implicit}), and studying \eqref{eq:main_problem} is a good starting point for understanding the behavior of networks learned via gradient descent even without explicit weight decay. Interestingly, minimum-norm interpolation corresponds to the \emph{rich regime}, and does not correspond to any kernel \citep{savarese2019infinite}.
For the aforementioned reasons, understanding the properties of min-norm interpolators has attracted much interest in recent years \citep{savarese2019infinite, ongie2019function, ergen2021convex, hanin2021ridgeless, debarre2022sparsest, boursier2023penalising}.
% \textcolor{red}{gradient descent does not exactly minimize the $\ell_2$ norm and the inductive bias characterization does not even exist \cite{?}. But it is known that min-norm networks already induce a rich inductive bias that goes beyond the kernel regime and, in fact, doesn't correspond to any kernel \cite{?}. Moreover, as we shall describe later, the interpolating solutions reached by gradient descent are qualitatively similar to the min-norm networks \citep{shevchenko2022mean}, and thus, studying \eqref{eq:main_problem} is a good starting point also for understanding the behavior of networks learned via gradient descent.} 

\paragraph{Noisy interpolation learning.} We consider a noisy distribution $\dist$ over $[0,1] \times \IR$:
\begin{equation} \label{eq:define_D}
    x \sim \unif([0,1])\;\;\;\; \text{ and }\;\;\;\; y=f^*(x)+\eps \; \text{ with } \eps \textrm{ independent of }\, x,
\end{equation}
where $x$ is uniform for simplicity and concreteness\footnote{All our results should also hold for any absolutely continuous distribution with bounded density and support. Roughly speaking, this can be achieved by dividing the support into disjoint intervals such that the distribution in each interval is well-approximated by a uniform distribution.}. The noise $\eps$ follows some arbitrary (but non-zero) distribution, and learning is based on an i.i.d.~training set $S\sim\dist^n$.  Since the noise is non-zero, the ``ground truth'' predictor $f^*$ has non-zero training error, seeking a training error much smaller than that of $f^*$ would be overfitting (fitting the noise) and necessarily cause the complexity (e.g.~norm) of the learned predictor to explode.  The ``right'' thing to do is to balance between the training error and the complexity $\norm{\theta}$.  Indeed, under mild assumptions, this balanced approach leads to asymptotic consistency, with $\hat{f}_S \xrightarrow{n\rightarrow\infty} f^* $ and the asymptotic population risk of $\hat{f}_S$ converging to the Bayes risk.  But what happens when we overfit and use the interpolating learning rule \eqref{eq:main_problem}?

\begin{figure}[t]  
 \begin{center} 
 \vspace{-5mm}\includegraphics[scale=0.35]{Figures/sp-min-norm2.pdf}
    \vspace{-2mm}\caption{Comparison between linear-spline (purple) and min-norm (green) interpolators.}
    \vspace{-5mm}
     \label{fig:min-norm-illustration1}
 \end{center}
 \end{figure}

\paragraph{Linear Splines.} At first glance, we might be tempted to think that two-layer ReLUs behave like linear splines (see Figure~\ref{fig:min-norm-illustration1}). Indeed, if minimizing the norm of weights $w_i$ and $a_i$ but {\em not} the biases $b_i$ in \eqref{eq:main_problem}, linear splines are a valid minimizer \citep{savarese2019infinite,ergen2021convex}. As the number of noisy training points increases, linear splines ``zig-zag'' with tighter ``zigs'' but non-vanishing ``amplitude'' around $f^*$, resulting in an interpolator which roughly behaves like $f^*$ plus some added non-vanishing ``noise''.  This does not lead to consistency, but is similar to a nearest-neighbor predictor (each prediction is a weighted average of two neighbors).  Indeed, in Theorem~\ref{thm:linear-splines} of Section~\ref{sec:linear-spline}, we show that linear splines exhibit ``tempered'' behavior, with asymptotic risk proportional to the noise level.

\paragraph{From Splines to Min-Norm ReLU Nets.} It turns out minimum norm ReLU networks, although piecewise linear, are not quite linear splines: roughly speaking, and as shown in Figure~\ref{fig:min-norm-illustration1}, they are more conservative in the number of linear ``pieces''. Because of this, in convex (conversely, concave) regions of the linear spline, minimum norm ReLU nets ``overshoot'' the linear spline in order to avoid breaking linear pieces. This creates additional ``spikes'', extending above and below the data points (see Figures~\ref{fig:min-norm-illustration1} and~\ref{fig:min-norm-illustration2}) and thus potentially increasing the error. In fact, such spikes are also observed in interpolants reached by gradient descent \citep[Figure 1]{shevchenko2022mean}. How bad is the effect of such spikes on the population risk? 

\subsection*{Our Contribution}\label{subsec:contributions}

\paragraph{Effect of Overfitting on $L_p$ Risk.} It turns out the answer is quite subtle and, despite considering the same interpolator, the nature of overfitting actually depends on how we measure the error. For a function $f:\IR \rightarrow\IR$, we measure its $L_p$ population error and the reconstruction error respectively as
$$\mathcal{L}_p(f) := \Exp_{(x,y) \sim \dist} [|f(x)-y|^p] \quad \text{ and } \quad \mathcal{R}_p(f) := \Exp_{x \sim \unif([0,1])} [|f(x)-f^*(x)|^p].$$
We show in Theorems~\ref{thm:tempered-for-ell_1} and~\ref{thm:tempered-for-ell_1-lower_bound} of Section~\ref{sec:tempered-L1} that for $1 \leq p < 2$, 
\begin{equation}\label{eq:intro_main}
    \mathcal{L}_p(\hat{f}_S)\xrightarrow{n\rightarrow\infty} \Theta \left( \frac{1}{(2-p)_+} \right) \, \mathcal{L}_p(f^*).
\end{equation}
This is an upper bound for any Lipschitz target $f^*$ and any noise distribution, and it is matched by a lower bound for Gaussian noise.  That is, for abs-loss ($L_1$ risk), as well as any $L_p$ risk for $1\leq p<2$, overfitting is {\bf tempered}. But this tempered behavior explodes as $p \rightarrow 2$, and we see a sharp transition. We show in Theorem~\ref{thm:ell2-catastrophic} of Section~\ref{sec:catastrophic} that for any $p\geq 2$, including for the square loss ($p=2$), in the presence of noise,
$\mathcal{L}_p(\hat{f}_S)\xrightarrow{n\rightarrow\infty} \infty$ and overfitting is {\bf catastrophic}. 


\paragraph{Convergence vs. Expectation.} The behavior is even more subtle, in that even for $1\leq p<2$, although the risk $\mathcal{L}_p(\hat{f}_S)$ converges in probability to a tempered behavior as in \eqref{eq:intro_main}, its {\em expectation} is infinite: $\Exp_S[\mathcal{L}_p(\hat{f}_S)]=\infty$.  Note that in studying tempered overfitting, \citet{mallinar2022benign} focused on this expectation, and so would have categorized the behavior as ``catastrophic'' even for $p=1$, emphasizing the need for more careful consideration of the effect of overfitting.  

\paragraph{I.I.D.~Samples vs. Samples on a Grid.} The catastrophic effect of interpolation on the $L_p$ risk with $p \geq 2$ is a result of the effect of fluctuations in the \textit{spacing} of the training points.  Large, catastrophic, spikes are formed by training points extremely close to their neighbors but with different labels (see Figures~\ref{fig:min-norm-illustration2} and~\ref{fig:bad-case-kink-main-text}). To help understand this, in Section~\ref{sec:grid} we study a ``fixed design'' variant of the problem, where the training inputs lie on a uniform grid, $x_i=i/n$, and responses follow $y_i=f^*(x_i)+\epsilon_i$. In this case, interpolation is always tempered, with $\mathcal{L}_p(\hat{f}_S)\xrightarrow{n\rightarrow\infty} O(  \mathcal{L}_p(f^*) )$ for any constant $p\geq 1$ (Theorem~\ref{thm:grid} of Section~\ref{sec:grid}).

\paragraph{Discussion and Takeaways.} 

Our work is the first to study noisy interpolation learning with min-norm ReLU networks for regression. It is also the first to study noisy interpolation learning in neural networks where the input dimension does not grow with the sample size, and to consider non-linearly-interpolatable data distributions (see below for a comparison with concurrent work in a classification setting). The univariate case might seem simplistic, but is a rich and well-studied model in its own right \citep{shevchenko2022mean,ergen2021convex,hanin2021ridgeless,debarre2022sparsest,boursier2023penalising,williams2019gradient,mulayoff2021implicit,safran2022effective}, and as we see, it already exhibits many complexities and subtleties that need to be resolved, and is thus a non-trivial necessary first step if we want to proceed to the multivariate case.

The main takeaway from our work is that the transition from tempered to catastrophic overfitting can be much more subtle than previously discussed, both in terms of the details of the setting (e.g., sampled data vs. data on a grid) and 
%even more so in 
in terms of
the definition and notion of overfitting (the loss function used, and expectation vs. high probability). Understanding these subtleties is crucial before moving on to more complex models.

More concretely, we see that for the square loss, the behavior does not fit the ``tempered overfitting'' predictions of ~\citet{mallinar2022benign}, and for the $L_1$ loss we get a tempered behavior with high probability but not in expectation, which highlights that the definitions of \citep{mallinar2022benign} need to be refined. We would of course not get such strange behavior with the traditional non-overfitting approach of balancing training error and norm; in this situation the risk converges almost surely to the optimal risk, with finite expectation and vanishing variances. Moreover, perhaps surprisingly, when the input data is on the grid (equally spaced), the behavior is tempered for all losses even in the presence of label noise. This demonstrates that the catastrophic behavior for $L_p$ losses for $p \geq 2$ is not just due to the presence of label noise; it is the combination of label noise and sampling of points that hurts generalization.
We note that previous works considered benign overfitting with data on the grid as a simplified setting, which may help in understanding more general situations \citep{beaglehole2022kernel,lai2023generalization}. Our results imply that this simplification might change the behavior of the interpolator significantly. In summary, the nature of overfitting is a delicate property of the combination of how we measure the loss and how training examples are chosen.

\paragraph{Comparison with concurrent work.}
In a concurrent and independent work, \citet{kornowski2023tempered} studied interpolation learning in univariate two-layer ReLU networks in a classification setting, and showed that they exhibit tempered overfitting. 
%Roughly speaking, 
In contrast to our regression setting,
in classification 
%as we sign threshold the output, 
only the output's sign affects generalization, and hence the height of 
the spikes 
%and input distribution 
do not play a significant role. As a result, 
our regression setting 
exhibits a fundamentally different behavior, and
the above discussion on the delicateness of the overfitting behavior in regression does not apply to their classification setting.
%offers fundamentally new insights 
%on the delicateness of the overfitting behavior. 
%% OLD PARAGRAPH, TO BE REMOVED
%Our work is a first step\footnote{We note that in a concurrent and independent work, \citet{kornowski2023tempered} showed tempered overfitting in univariate ReLU networks in a classification setting.} toward studying noisy interpolation learning 
%in neural networks where input dimension does not grow with the sample size, and the first to consider non-linearly-interpretable data distributions.
%on non-linearly-interpolatable data in actual neural networks, where the capacity of the model comes from the size of the network and not the dimension of the data.  
%We study the univariate case. Univariate regression with min-norm ReLU networks is a rich model in its own right \citep[e.g.][]{savarese2019infinite,ergen2021convex,hanin2021ridgeless,debarre2022sparsest,boursier2023penalising,williams2019gradient,mulayoff2021implicit,safran2022effective} and a starting point for further investigation. 

%While understanding the overfitting nature of min-norm neural networks is already of significant interest, our work has several important takeaways. We have to be careful when studying and discussing overfitting. \citet{mallinar2022benign} made general predictions that neural networks exhibit tempered behavior after some experiments and also explained this behavior with some heuristic argument. We see that for universally studied squared loss, the behavior of this most natural neural-network learning rule does not fit the ``tempered overfitting'' predictions of ~\citet{mallinar2022benign}. Even for $L_1$ loss, we get a temepred behavior with high probability but not in expectation.  A part of the contribution is to highlight that the definitions of \citep{mallinar2022benign} need to be refined. 

%Moreover, perhaps surprisingly, when the input data is on the grid (equally spaced), the behavior is tempered for all losses even in the presence of label noise. This demonstrates that the catastrophic behavior for $L_p$ losses for $p \geq 2$ is not just due to the presence of label noise; it is the combination of label noise and sampling of points that hurts generalization.  Understanding these issues in detail is crucial before progressing to more complex situations. We note that previous works considered benign overfitting with data on the grid as a simplified setting, which may help in understanding more general situations \citep{beaglehole2022kernel,lai2023generalization}. Our results imply that this simplification might change the behavior of the interpolator significantly.

 
 \begin{figure}[t]
     \begin{center}
     \vspace{-5mm}
\includegraphics[scale=0.4]{Figures/large_points.pdf}
   \vspace{-2mm}  \caption{The min-norm interpolator for $30$ random points with $f^* \equiv 0$ and $\normal(0,1)$ label noise.}
     \label{fig:min-norm-illustration2}
     \vspace{-5mm}
\end{center}
 \end{figure}
 
\section{Review: Min-Norm ReLU Networks} \label{sec:review_min_norm_nets}

Minimum-norm unbounded-width univariate two-layer ReLU networks have been extensively studied in recent years, starting with \citet{savarese2019infinite}, with the exact formulation \eqref{eq:main_problem} incorporating a skip connection due to \citet{boursier2023penalising}.   \citeauthor{boursier2023penalising}, following prior work, establish that a minimum of \eqref{eq:main_problem} exists, with a finite number of units, and that it is also unique.  

The problem in \eqref{eq:main_problem} is also equivalent to minimizing the ``representation cost'' $
    R(f) = \int_{\IR} \sqrt{1+x^2}|f''(x)| dx $
over all interpolators $f$, although we will not use this characterization explicitly in our analysis. Compared to \citet{savarese2019infinite}, where the representation cost is given by $\max\{\int |f''(x)| dx, |f'(-\infty)+f'(+\infty)|\}$, the weighting $\sqrt{1+x^2}$ is due to penalizing the biases $b_i$.  More significantly, the skip connection in \eqref{eq:net} avoids the ``fallback'' terms of $|f'(-\infty)+f'(+\infty)|$, which only kick-in in extreme cases (very few points or an extreme slope).  This simplified the technical analysis and presentation, while rarely affecting the solution.  

\citeauthor{boursier2023penalising} provide the following characterization of the minimizer\footnote{
If the biases $b_i$ are {\em not} included in the norm $\norm{\theta}$ in \eqref{eq:main_problem}, and this norm is replaced with $\sum_i(a_i^2+w_i^2)$, the modified problem admits multiple non-unique minimizers, including a linear spline (with modified behavior past the extreme points) \citep{savarese2019infinite}.  This set of minimizers was characterized by \citet{hanin2021ridgeless}.  Interestingly, the minimizer $\hat{f}_S$ of \eqref{eq:main_problem} (when the biases are included in the norm) is also a minimizer of the modified problem (without including the biases).  All our results apply also to the setting without penalizing the biases in the following sense: the upper bounds are valid for all minimizers, while some minimizer, namely $\hat{f}_S$ that we study, exhibits the lower bound behavior.} $\hat{f}_S$ of \eqref{eq:main_problem}, which we will rely on heavily:
\begin{lemma}[\citet{boursier2023penalising}]\label{lem:char}
    For $0 \leq x_1<x_2<\cdots<x_n$, the problem in \eqref{eq:main_problem} admits a unique minimizer of the form:
    \begin{equation} \label{eq:min-norm_interpolator}
        \hat{f}_S(x) = ax + b + \sum_{i=1}^{n-1} a_i (x - \tau_i)_+~,
    \end{equation}
    where $\tau_i \in [x_i,x_{i+1})$ for every $i \in [n-1]$. 
\end{lemma}
As in the above characterization, it is very convenient to take the training points to be sorted.  Since the learned network $\hat{f}_S$ does not depend on the order of the points, we can always ``sort'' the points without changing anything.  And so, throughout the paper, we will always take the points to be sorted (formally, the results apply to i.i.d.~points, and the analysis is done after sorting these points).  


\section{Warm up: tempered overfitting in linear-spline interpolation} \label{sec:linear-spline}

We start by analyzing tempered overfitting for linear-spline interpolation. Namely, we consider the piecewise-linear function obtained by connecting each pair of consecutive points in the dataset $S \sim \dist^n$ (see Figures~\ref{fig:min-norm-illustration1} and \ref{fig:splines-main_text} left) and analyze its test performance. %The linear-spline interpolator (after extending linear pieces beyond the endpoints, as we will discuss in Section~\ref{sec:delicate}),
%is a minimizer of the network's norms in a setting where the bias terms are not penalized, albeit not a unique minimizer \citep{savarese2019infinite,ergen2021convex,hanin2021ridgeless}. In our setting, the linear-spline interpolator does not minimize the network's norms, but analyzing its test performance is a useful first step toward understanding min-norm interpolation.

\begin{figure}[t]
\begin{center}
\vspace{-5mm}
\hspace{1cm}
\includegraphics[scale=0.6]{Figures/splines2.pdf}
\vspace{-0.9cm}
\caption{An illustration of the linear spline interpolator $\hat{g}_S$ (left), and of the variant $\hat{h}_S$ where linear pieces are extended beyond the endpoints (right).}
\vspace{-5mm}
\label{fig:splines-main_text}
\end{center}
\end{figure}

Given a dataset $S = \{(x_i,y_i)\}_{i=1}^n$, let $g_i:\IR \rightarrow \IR$ be the affine function joining the points $(x_{i},y_{i})$ and $(x_{i+1},y_{i+1})$. Thus, $g_i$ is the straight line joining the endpoints of the $i$-th interval. Then, the linear spline interpolator $\hat{g}_S: [0,1] \rightarrow \IR$ is given by
\begin{equation}\label{eq:linear-spline}
   \hat{g}_S(x) := y_1 \cdot \mathbf{1}\{ x < x_1\} + y_n \cdot \mathbf{1}\{x \geq x_{n}\}+\sum_{i=1}^{n-1} g_i(x)\cdot \mathbf{1}\{x\in [x_{i},x_{i+1})\}. 
\end{equation}
Note that in the intervals $[0,x_1]$ and $[x_n,1]$ the linear-spline $\hat{g}_S$ is defined to be constants that correspond to labels $y_1$ and $y_n$ respectively. The following theorem characterizes the asymptotic behavior of $\mathcal{L}_p(\hat{g}_S)$ for every $p \geq 1$:

\begin{theorem}\label{thm:linear-splines}
    Let $f^*$ be any Lipschitz function and $\dist$ be the distribution from \eqref{eq:define_D}. Let $S \sim \dist^{n}$, and $\hat{g}_S$ be the linear-spline interpolator (\eqref{eq:linear-spline}) w.r.t. the dataset $S$. Then, for any $p \geq 1$ there is a constant $C_p$ such that       
    \begin{equation*} \label{eq:spline-ub}
        \lim_{n \rightarrow \infty} \Pr_S  \left[\mathcal{R}_p(\hat{g}_S) \leq C_p\, \mathcal{L}_p(f^*) \right] = 1 \quad \text{ and }  \quad  \lim_{n \rightarrow \infty} \Pr_S  \left[\mathcal{L}_p(\hat{g}_S) \leq C_p\, \mathcal{L}_p(f^*) \right] = 1.
    \end{equation*}
\end{theorem}

The theorem shows that the linear-spline interpolator exhibits tempered behavior, namely, w.h.p. over $S$ the interpolator $\hat{g}_S$ performs like the predictor $f^*$, up to a constant factor. To understand why Theorem~\ref{thm:linear-splines} holds, note that for all $i \in [n-1]$ and $x \in [x_i,x_{i+1}]$ the linear-spline interpolator satisfies $\hat{g}_S(x) \in [\min\{y_i,y_{i+1}\}, \max\{y_i,y_{i+1}\}]$. Moreover, we have for all $i \in [n]$ that $|y_i-f^*(x_i)| = |\epsilon_i|$, where $\epsilon_i$ is the random noise. Using these facts, it is not hard to bound the expected population loss of $\hat{g}_S$ in each interval $[x_i,x_{i+1}]$, and by using the law of large numbers it is also possible to bound the probability (over $S$) that the loss in the 
domain $[0,1]$ is large. Thus, we can bound the $L_p$ loss both in expectation and in probability.

\paragraph{Delicate behavior of linear splines.} We now consider the following variant of the linear-spline interpolator:
\begin{equation}\label{eq:hhat}
   \hat{h}_S(x) := g_1(x) \cdot \mathbf{1}\{ x < x_1\} + g_{n-1}(x) \cdot \mathbf{1}\{x > x_{n}\}+ \hat{g}_S(x) \cdot \mathbf{1}\{x\in [x_{1},x_{n}]\}. 
\end{equation}
In words, $\hat{h}_S$ is exactly the same as $\hat{g}_S$ in the interval $[x_1,x_n]$, but it extends the linear pieces $g_1$ and $g_{n-1}$ beyond the endpoints $x_1$ and $x_n$ (respectively), as illustrated in Figure~\ref{fig:splines-main_text} (right). The interpolator $\hat{h}_S$ still exhibits tempered behavior in probability, similarly to $\hat{g}_S$. However, perhaps surprisingly, $\hat{h}_S$ is not tempered in expectation (see Appendix \ref{sec:delicate} for details). This delicate behavior of the linear-spline interpolator is important since in the next section we will show that the min-norm interpolator has a similar behavior to $\hat{h}_S$ in the intervals $[0,x_1],[x_n,1]$, and as a consequence, it is tempered with high probability but not in expectation.
\section{Min-norm interpolation with random data} \label{sec:main_results} 

In this section, we study the performance of the min-norm interpolator with random data. We first present some important properties of the min-norm interpolator in Section~\ref{sec:characterizing}. In Sections~\ref{sec:tempered-L1} and~\ref{sec:catastrophic} we use this characterization to study its performance.

\subsection{Characterizing the min-norm interpolator} \label{sec:characterizing}

Our goal is to give a characterization of the min-norm interpolator $\hat{f}_S(x)$ (\eqref{eq:min-norm_interpolator}), in terms of linear splines as defined in \eqref{eq:linear-spline}. Recall the definition of affine functions $g_1(x),\dots, g_{n-1}(x)$, which are piece-wise affine functions joining consecutive points. Let $\delta_i$ be the slope of the line $g_i(x)$, i.e. $\delta_i=g_i'(x)$. We denote $\delta_0:=\delta_1$ and $\delta_n:=\delta_{n-1}$. Then, we can define the sign of the curvature of the linear spline $\hat{g}_S(x)$ at each point.

\begin{definition}\label{def:discrete-curvature}
    For any $i\in [n]$,
      $$ \curv(x_i) = \begin{cases}
  +1  & \delta_i > \delta_{i-1} \\
  0 & \delta_i = \delta_{i+1} \\
  -1 & \delta_i < \delta_{i-1}
\end{cases}$$
\end{definition}

\begin{figure}[t]
\begin{center}
 \vspace{-5mm}   
\includegraphics[scale=0.6]{Figures/min-norm-illus.pdf}
\vspace{-0.5cm}
\caption{An illustration of the characterization of $\hat{f}_S$ from Lemma~\ref{lem:complete-description-property-main_text}.}
\label{fig:geometric-illustration-of-triangle-main_text}
\vspace{-3mm}
\end{center}
\end{figure}
Based on the curvature, the following lemma geometrically characterizes $\hat{f}_S$ in any interval $[x_i,x_{i+1})$, in terms of the linear pieces $g_{i-1},g_i,g_{i+1}$.

\begin{lemma}\label{lem:complete-description-property-main_text}
The function $\hat{f}_S$ can be characterized as follows:
        \begin{itemize}
        \item $\hat{f}_S(x) =g_1(x)$ for $x\in (-\infty, x_2)$;
        \item $\hat{f}_S(x) =g_{n-1}(x)$ for $x \in [x_{n-1},\infty)$;
        \item In each interval $[x_i,x_{i+1})$ for $i \in \{2, \dots n-2\}$, 
        \begin{enumerate}
            \item If $\curv(x_i)=\curv(x_{i+1})=+1$ then
        $$ \max\{g_{i-1}(x), g_{i+1}(x)\} \leq  \hat{f}_S (x) \leq g_i(x);$$
        \item  If $\curv(x_i)=\curv(x_{i+1})=-1$ then
        $$  \min\{g_{i-1}(x), g_{i+1}(x)\} \geq  \hat{f}_S (x) \geq  g_i(x);$$ 
        \item Else, i.e. either $\curv(x_i)=0$ or $\curv(x_{i+1})=0$ or $\curv(x_{i}) \neq \curv(x_{i+1})$,
        $$\hat{f}_S(x)=g_i(x).$$
        \end{enumerate}
        \end{itemize}
\end{lemma}
The lemma implies that $\hat{f}_S$ coincides with $\hat{g}_S$ except in an interval $[x_i,x_{i+1})$ where the curvature of the two points are both $+1$ or $-1$ (see Figure~\ref{fig:geometric-illustration-of-triangle-main_text}). Intuitively, this property captures the worst-case effect of the spikes and will be crucial in showing the tempered behavior of $\hat{f}_S$ w.r.t. $L_p$ for $p\in [1,2)$. However, this still does not imply that such spikes are necessarily formed. 

To this end, \citet[Lemma 8]{boursier2023penalising} characterized the situation under which indeed these spikes are formed. Roughly speaking, if the sign of the curvature changes twice within three points, then we get a spike. Formally, we identify special points from left to right recursively where the sign of the curvature changes.
\begin{definition}\label{def:cruv-changed}
    We define $n_1:=1$. Having defined the location of the special points $n_1,\dots, n_{i-1}$, we recursively define 
    $$n_i= \min \{ j>n_{i-1} : \curv(x_{j}) \neq \curv (x_{n_i})\}.$$
    If there is no such $n_{i-1} < j \leq n$ where $\curv(x_{j}) \neq \curv (x_{n_i})$, then $n_{i-1}$ is the location of the last special point.
\end{definition}

\begin{lemma}[\citet{boursier2023penalising}]\label{lem:sparsity-main_text}
    For any $k \geq 1$, if $\delta_{n_k -1 }  \neq  \delta_{n_k}$ and $n_{k+1}= n_k + 2$, then $\hat{f}_S$ has exactly one kink between $(x_{{n_k}-1}, x_{n_{k+1}})$. Moreover, if $\curv(x_{n_k})=\curv(x_{n_k+1})=-1$ then $\hat{f}_S(x)=\min\{g_{n_k-1}(x), g_{n_k+1}(x)\}$ in $[x_{n_k},x_{n_k+1})$.
\end{lemma}

\begin{figure}[t] 
\vspace{-5mm}
\begin{center}  
\hspace{1cm}\includegraphics[scale=0.65]{Figures/configuration.pdf}
\vspace{-8mm}
\caption{An illustration of the spike formed by Lemma~\ref{lem:sparsity-main_text}. Here, $x_2$ and $x_4$ are two consecutive special points with exactly one point in between. There must be exactly one kink in $(x_1,x_4)$. Thus, in $[x_2,x_3)$, the  interpolator $\hat{f}_S$ must be $\min\{g_1(x),g_3(x)\}$.}
\label{fig:bad-case-kink-main-text}
\vspace{-3mm}
\end{center}
\end{figure}

This is a slight variation of \citep[Lemma 8]{boursier2023penalising}, which we reprove in the appendix for completeness. See Figure~\ref{fig:bad-case-kink-main-text} for an illustration of the above lemma.
To show the catastrophic behavior of $\hat{f}_S$ for $p \geq 2$, we will consider events under which such configurations of points are formed. This will result in spikes giving catastrophic behavior. 

\subsection{Tempered overfitting for \texorpdfstring{$L_p$}{TEXT} with \texorpdfstring{$p \in [1,2)$}{TEXT}}\label{sec:tempered-L1}

We now show the tempered behavior of the minimal norm interpolator w.r.t. $L_p$ losses for $p \in [1,2)$.
\begin{theorem} \label{thm:tempered-for-ell_1}
Let $f^*$ be a Lipschitz function and $\dist$ be the distribution from \eqref{eq:define_D}. Sample $S\sim \dist^n$, and let $\hat{f}_S$ be the min-norm interpolator (\eqref{eq:min-norm_interpolator}). Then, for some universal constant $C > 0$, for any $p \in [1,2)$ we have 
\[
  \lim_{n \rightarrow \infty} \Pr_S \left[\mathcal{R}_p(\hat{f}_S) \leq \frac{C}{2-p} \cdot \,  \mathcal{L}_p(f^*) \right] = 1 \quad \text{and} \quad   \lim_{n \rightarrow \infty} \Pr_S \left[\mathcal{L}_p(\hat{f}_S) \leq \frac{C}{2-p} \cdot \,  \mathcal{L}_p(f^*) \right] = 1~.
\]
\end{theorem}
The proof of Theorem~\ref{thm:tempered-for-ell_1} builds on Lemma~\ref{lem:complete-description-property-main_text}, which implies that in an interval $[x_i,x_{i+1})$, a spike in the interpolator $\hat{f}_S$ must be bounded within the triangle obtained from $g_{i-1},g_i,g_{i+1}$ (see Figure~\ref{fig:geometric-illustration-of-triangle-main_text}). Analyzing the population loss of $\hat{f}_S$ requires considering the distribution of the spacings between data points. Let $\ell_0,\ldots,\ell_n$ be such that 
\begin{equation} \label{eq:define_ell}
    \forall i \in [n-1]\;\; \ell_i = x_{i+1}-x_i, \;\;\;\; \ell_0 = x_1, \;\;\;\; \ell_n = 1-x_n~.
\end{equation}
Prior works \citep{alagar1976distribution,pinelis2019order} established that  
\begin{equation} \label{eq:ell_distribution}
    \left( \ell_0,\dots,\ell_n \right) \sim  \left( \frac{X_0}{X}, \dots, \frac{X_n}{X} \right), \text{ where } X_0,\dots,X_n \iid \text{Exp}(1), \text{ and } X:=\sum_{i=0}^{n} X_i~.
\end{equation}
The slopes of the affine functions $g_{i-1},g_{i+1}$ are roughly $\frac{1}{\ell_{i-1}},\frac{1}{\ell_{i+1}}$, where $\ell_j$ are the lengths as defined in \eqref{eq:define_ell}. Hence, the spike's height is proportional to $\frac{\ell_i}{\max\{\ell_{i-1},\ell_{i+1}\}}$. As a result, the $L_p$ loss in the interval $[x_i,x_{i+1}]$ is roughly 
\[
    \left(\frac{\ell_i}{\max\{\ell_{i-1},\ell_{i+1}\}} \right)^p \cdot \ell_i = \frac{\ell_i^{p+1}}{\max\{\ell_{i-1},\ell_{i+1}\}^p}~.
\]
Using the distribution of the $\ell_j$'s given in \eqref{eq:ell_distribution}, we can bound the expectation of this expression. Then, similarly to our discussion on linear splines in Section~\ref{sec:linear-spline}, in the range $[x_1,x_n]$ we can bound the $L_p$ loss both in expectation and in probability. In the intervals $[0,x_1]$ and $[x_n,1]$, the expected loss is infinite (similarly to the interpolator $\hat{h}_S$ in \eqref{eq:hhat}), and therefore we have 
\begin{equation} \label{eq:L1_infinite_exp}
    \Exp_S \left[\mathcal{L}_p(\hat{f}_S) \right] = \infty~.
\end{equation}
Still, we can get a high probability upper bound for the $L_p$ loss in the intervals $[0,x_1]$ and $[x_n,1]$. Thus, we get a bound on $L_p$ loss in the entire domain $[0,1]$ w.h.p. We note that the definition of tempered overfitting in \citet{mallinar2022benign} considers only the expectation. Theorem~\ref{thm:tempered-for-ell_1} and \eqref{eq:L1_infinite_exp} imply that in our setting we have tempered behavior in probability but not in expectation, which demonstrates that tempered behavior is delicate.

We also show a lower bound for the population loss $L_p$ which matches the upper bound from Theorem~\ref{thm:tempered-for-ell_1} (up to a constant factor independent of $p$). The lower bound holds already for $f^* \equiv 0$ and Gaussian label noise.

\begin{theorem} \label{thm:tempered-for-ell_1-lower_bound}
Let $f^* \equiv 0$, consider label noise $\epsilon \sim \normal(0,\sigma^2)$ for some constant $\sigma>0$, and let
$\dist$ be the corresponding distribution from \eqref{eq:define_D}. Let $S\sim \dist^n$, and let $\hat{f}_S$ be the min-norm interpolator (\eqref{eq:min-norm_interpolator}). Then, for some universal constant $c > 0$, for any $p \in [1,2)$ we have 
\[
   \lim_{n \rightarrow \infty} \Pr_S \left[\mathcal{R}_p(\hat{f}_S) \geq \frac{c}{2-p} \cdot \mathcal{L}_p(f^*)  \right] = 1 \quad \text{and} \quad \lim_{n \rightarrow \infty} \Pr_S \left[\mathcal{L}_p(\hat{f}_S) \geq \frac{c}{2-p} \cdot \mathcal{L}_p(f^*)  \right] = 1~.
\]
\end{theorem}

The proof of the above lower bound follows similar arguments to the proof of catastrophic overfitting for $p \geq 2$, which we will discuss in the next section.

\subsection{Catastrophic overfitting for \texorpdfstring{$L_p$}{TEXT} with \texorpdfstring{$p \geq 2$}{TEXT}} \label{sec:catastrophic}

Next, we prove that for the $L_p$ loss with $p \geq 2$, the min-norm interpolator exhibits catastrophic overfitting. We prove this result already for $f^* \equiv 0$ and Gaussian label noise:

\begin{theorem}\label{thm:ell2-catastrophic}
    Let $f^* \equiv 0$, consider label noise $\epsilon \sim \normal(0,\sigma^2)$ for some constant $\sigma>0$, and let $\dist$ be the corresponding distribution from \eqref{eq:define_D}.
    Let $S \sim \dist^n$, and let $\hat{f}_S$ be the min-norm interpolator (\eqref{eq:min-norm_interpolator}).
    Then, for any $p \geq 2$ and $b>0$,
    \[
       \lim_{n \to \infty} \Pr_S\left[{\mathcal{R}_p(\hat{f}_S) > b} \right] = 1 \quad \text{and} \quad \lim_{n \to \infty} \Pr_S\left[{\mathcal{L}_p(\hat{f}_S) > b} \right] = 1~.
    \]
\end{theorem}

To obtain some intuition on this phenomenon, consider the first four samples $(x_1,y_1),\ldots,(x_4,y_4)$, and let $\ell_i$ be the lengths of the intervals as defined in \eqref{eq:define_ell}. We show that with constant probability, 
the configuration of the labels of these samples satisfies certain properties, which are illustrated in Figure~\ref{fig:bad-case-kink-main-text}.
In this case, Lemma~\ref{lem:sparsity-main_text} implies that in the interval $[x_2,x_3]$ the interpolator $\hat{f}_S$ is equal to $\min\{g_1(x),g_3(x)\}$, where $g_1$ (respectively, $g_3$) is the affine function that connects $x_1,x_2$ (respectively, $x_3,x_4$). Now, as can be seen in the figure, in this ``unfortunate configuration'' the interpolator $\hat{f}_S$ spikes above $f^* \equiv 0$ in the interval $[x_2,x_3]$, and the spike's height is proportional to $\frac{\ell_2}{\max\{\ell_1,\ell_3\}}$. As a result, the $L_p$ loss in the interval $[x_2,x_3]$ is roughly $\frac{\ell_2^{p+1}}{\max\{\ell_1,\ell_3\}^p}$. Using \eqref{eq:ell_distribution}, we can show that 
$\Exp_S \left[ \frac{\ell_2^{p+1}}{\max\{\ell_1,\ell_3\}^p} \right] = \infty$ for any $p \geq 2$.

We then divide divide the $n$ samples in $S$ into $\Theta(n)$ disjoint subsets and consider the events that labels are such that the $4$ middle points exhibit an ``unfortunate configuration'' as described above. Using the fact that we have $\Theta(n)$ such subsets and the losses in these subsets are only mildly correlated, we are able to prove that $\hat{f}_S$ exhibits a catastrophic behavior also in probability.

We note that the proof of Theorem~\ref{thm:tempered-for-ell_1-lower_bound} follows similar arguments, except that when $p<2$ the expectation of the $L_p$ loss in each subset with an ``unfortunate configuration'' is finite, and hence we get a finite lower bound.

\section{Min-norm interpolation with samples on the grid} \label{sec:grid}

In this section, we analyze the population loss of the min-norm interpolator, when the $n$ data-points in $S$ are uniformly spaced, instead of i.i.d. uniform sampling considered in the previous sections. Namely, consider
the training set $S=\{(x_i,y_i): i \in [n] \}$, where
\begin{equation} \label{eq:grid-data}
    x_i=\frac{i}{n} \hspace{2mm} \text{and} \hspace{2mm} y_i=f^*(x_i)+\eps_i \; 
    \text{ for i.i.d. noise } \; \eps_i~. 
\end{equation}
Note that the randomness in $S$ is only in the label noises $\epsilon_i$. 
It can be interpreted as a \emph{non-adaptive active learning} setting, where the learner can actively choose the training points, and then observe noisy measurements at these points, and the query points are selected on an equally spaced grid. We show that in this situation the min-norm interpolator exhibits tempered overfitting with respect to any ${L}_p$ loss:
\begin{theorem}\label{thm:grid}
 Let $f^*$ be any Lipschitz function. For the size-$n$ dataset $S$ given by \eqref{eq:grid-data}, let $\hat{f}_S$ be the min-norm interpolator (\eqref{eq:min-norm_interpolator}). Then for any $p\geq 1$, there is a constant $C_p$ such that
 \[
    \lim_{n \rightarrow \infty} \Pr_S \left[\mathcal{R}_p(\hat{f}_S) \leq C_p \, \mathcal{L}_p(f^*)\right] = 1 \quad \text{and} \quad \lim_{n \rightarrow \infty} \Pr_S \left[\mathcal{L}_p(\hat{f}_S) \leq C_p \, \mathcal{L}_p(f^*)\right] = 1~.
 \]
\end{theorem}

An intuitive explanation is as follows. Since the points are uniformly spaced, whenever spikes are formed, they can at most reach double the height without the spikes. Thus, the population loss of $\hat{f}_S(x)$ becomes worse but only by a constant factor. 
We remark that in this setting the min-norm interpolator exhibits tempered overfitting both in probability (as stated in Theorem~\ref{thm:grid}) and in expectation. From Theorem~\ref{thm:grid} we conclude that the catastrophic behavior for $L_p$ with $p \geq 2$ shown in Theorem~\ref{thm:ell2-catastrophic}
stems from the non-uniformity in the lengths of the intervals $[x_i,x_{i+1}]$, which occurs when the $x_i$'s are drawn at random. 

% \section{Conclusion and Future Work}
% We study the overfitting nature of minimum $\ell_2$ norm, depth two ReLU networks in the noisy univariate regression setting. Our work suggests that the overfitting behavior is an extremely delicate property and more systematic evaluation criteria, experiments, and definitions are required as little things matter.   

==> gird.tex <==
\section{Regression setting for the Grid case}

Let $f^*:[0,1]\rightarrow \IR$ be $G$-Lipschitz.
%, i.e. $\lip{f^*}=G$. 
Consider the 
%following joint 
distribution $(x,y) \sim \dist$ on 
%space $(\mathcal{X} \times \mathcal{Y})=[0,1] \times \IR$. 
$[0,1] \times \IR$, such that
%The marginal 
$x \sim \unif([0,1])$ and $y=f^*(x)+\eps$, where $\eps\sim \normal(0,\sigma^2)$ for a fixed constant $\sigma > 0$.

%As a warm-up, we first
First, we
analyze the expected risk of the predictor we may get by training on the dataset $S=\{(x_i,y_i): i\in \{0,\dots,n\} \}$, where the $x_i$'s come from the grid on $[0,1]$ with uniform spacing between the points. 
%In particular, consider the following way of generating 
Namely, consider
the training set $S=\{(x_i,y_i): i=0,1,\dots n \}$, where
\begin{equation} \label{eq:grid-data}
    x_i=\frac{i}{n} \hspace{2mm} \text{and} \hspace{2mm} y_i=f^*(x_i)+\eps_i, \hspace{5mm} \text{where } \eps_i \sim \normal(0,\sigma^2)~.
\end{equation}
Note that the randomness here is only in the labels. 
 
For a function $f$, we denote
$L_p(f)=\Exp_{(x,y)\sim \dist} [|f(x)-y|^p]$. %Then, the worst-case risk w.r.t. $L_p$ of a predictor in $\ridgeless(S)$ is given by
%\[
%    L_p(\hat{f}_0)= \Exp_S \sup_{f \in \ridgeless(S)} [L_p(f)]~.
%\]
 \begin{theorem} 
 For the training set from \eqref{eq:grid-data} and any $p \in \IN_{+}$, we have
 \[
 \lim_{n \rightarrow \infty} \Exp_S \sup_{\hat{f} \in \ridgeless(S)} [L_p(\hat{f})] \leq 18^p \, L_p^*~,
 \]
 where $L_p^*=L_p(f^*)$ is the Bayes error.
\end{theorem}
\begin{proof}
First, we observe that the distance between two consecutive $x_i$'s is $1/n$. The domain $[0,1]$ is divided into $n$ intervals of length $1/n$. Let $g_i: \IR \rightarrow \IR$ be the affine function 
%which is just 
given by the straight line joining the endpoints of the $i$-th interval $(x_{i-1},y_{i-1})$ and $(x_i,y_i)$ for every $i\in[n]$. 

\nirmit{The following could actually be a lemma because it is helpful in almost all proofs. It requires some casework also to prove.}
Fix any $i\in \{2,\dots,n-1\}$, and consider $x\in [x_{i-1},x_i]$:
%$ \min\{ g_i(x), \min\{g_{i+1}(x) , g_{i-1}(x)\}\} \leq \hat{f}(x) \leq \max\{ g_i(x), \min\{g_{i+1}(x) , g_{i-1}(x)\}\}$ \\
 \[
 |\hat{f}(x)-f^*(x)| \leq \max\left\{ |g_i(x)-f^*(x)|, \min\{|g_{i+1}(x)-f^*(x)|, |g_{i-1}(x)-f^*(x)|\}\right\}~,
 \]
 and for $i\in\{1,n\}:$
 \[ 
 |\hat{f}(x)-f^*(x)| = |g_i(x)-f^*(x)|~.
 \]
 We can simplify each one by one.
\begin{align*}
 |g_i(x)-f^*(x)|=&\left| y_{i-1}+ \frac{(y_{i}-y_{i-1})}{x_{i}-x_{i-1}} (x-x_{i-1})-f^*(x)\right|\\
 =& \left| f^*(x_{i-1})+\eps_{i-1} + \frac{f^*(x_i)+\eps_i-f^*(x_{i-1})-\eps_{i-1}}{x_{i}-x_{i-1}}(x-x_{i-1}) -f^*(x)\right| \\
 \leq & \left| f^*(x_{i-1}) -f^*(x)\right|+ |\eps_{i-1}|+ \left( \frac{G/n+|\eps_i|+|\eps_{i-1}|}{1/n} \right)\cdot  \left| (x-x_{i-1}) \right| \\
 \leq & \frac{G}{n}+ |\eps_{i-1}|+ \left( \frac{G/n+|\eps_i|+|\eps_{i-1}|}{1/n} \right) \cdot \frac{1}{n} \\
 = &\frac{2G}{n}+ |\eps_i|+2 |\eps_{i-1}|.
\end{align*}
Similarly,
\begin{align*}
 |g_{i-1}(x)-f^*(x)|=&\left| y_{i-1}+ \frac{(y_{i-1}-y_{i-2})}{x_{i-1}-x_{i-2}} (x-x_{i-1})-f^*(x)\right|\\
 =& \left| f^*(x_{i-1})+\eps_{i-1} + \frac{f^*(x_{i-1})+\eps_{i-1}-f^*(x_{i-2})-\eps_{i-2}}{x_{i-1}-x_{i-2}}(x-x_{i-1}) -f^*(x)\right| \\
 \leq & \left| f^*(x_{i-1}) -f^*(x)\right|+ |\eps_{i-1}|+ \left( \frac{G/n+|\eps_{i-1}|+|\eps_{i-2}|}{1/n} \right) \left| (x-x_{i-1}) \right| \\
 \leq & \frac{G}{n}+ |\eps_{i-1}|+ \left( \frac{G/n+ |\eps_{i-1}|+|\eps_{i-2}|}{1/n} \right)\cdot \frac{1}{n} \\
 = &\frac{2G}{n}+ 2|\eps_{i-1}|+|\eps_{i-2}|.
\end{align*}

Using a similar strategy, we also bound:
\begin{align*}
 |g_{i+1}(x)-f^*(x)|=&\left| y_{i}+ \frac{(y_{i+1}-y_{i})}{x_{i+1}-x_{i}} (x-x_{i})-f^*(x)\right|\\
 =& \left| f^*(x_{i})+\eps_{i} + \frac{f^*(x_{i+1})+\eps_{i+1}-f^*(x_{i})-\eps_{i}}{x_{i+1}-x_{i}}(x-x_{i}) -f^*(x)\right| \\
 \leq & \left| f^*(x_{i}) -f^*(x)\right|+ |\eps_{i}|+ \left( \frac{G/n+|\eps_{i+1}|+|\eps_{i}|}{1/n} \right) \left| (x-x_{i-1}) \right| \\
 \leq & \frac{G}{n}+ |\eps_{i}|+ \left( \frac{G/n+|\eps_{i+1}|+|\eps_{i}|}{1/n} \right) \cdot \frac{1}{n}\\
 = &\frac{2G}{n}+ 2|\eps_{i}|+|\eps_{i+1}|.
\end{align*}
Therefore, combining the above three, for $x$ in the intermediate intervals:
\begin{align*}
    |\hat{f}(x)-f^*(x)| &\leq \max\left\{\frac{2G}{n}+2|\eps_{i-1}|+|\eps_i|, \frac{2G}{n}+2|\eps_{i-1}|+|\eps_{i-2}|,\frac{2G}{n}+2|\eps_i|+|\eps_{i+1}|\right\} \\
    & \leq \frac{2G}{n}+2|\eps_i|+2|\eps_{i-1}|+|\eps_{i-2}|+|\eps_{i+1}|~.
\end{align*}

Therefore,
\begin{align}
  \Exp_{x\sim \unif([0,1])} \left[ |\hat{f}(x)-f^*(x)|^p \right] &= \sum_{i=1}^{n} \prob{x\in [x_{i-1},x_i)} \Exp \left[|\hat{f}(x)-f^*(x)|^p \mid x\in [x_{i-1},x_i) \right]  \nonumber\\
  & \leq \frac{1}{n} \Big[ \underbrace{\left(\frac{2G}{n}+2|\eps_0|+|\eps_1|\right)^p}_{:=T_1}+ \underbrace{\sum_{i=2}^{n-1} \left( \frac{2G}{n}+2|\eps_i|+2|\eps_{i-1}|+|\eps_{i-2}|+|\eps_{i+1}| \right)^p}_{:=T_2} \nonumber\\
  & + \underbrace{\left(\frac{2G}{n}+2|\eps_{n-1}|+|\eps_{n}| \right)^p}_{:=T_3}  \Big] \label{eq:grid-three-terms}
 % &\leq \frac{2^p}{n} \sum_{i=1}^{n} \left( (|\eps_i|+|\eps_{i-1}|+|\eps_{i-2}|+|\eps_{i+1}|)^p + \sum_{j=1}^{p} \binom{p}{j} \left(\frac{G}{n}\right)^j (|\eps_i|+2|\eps_{i-1}|+|\eps_{i-2}|+|\eps_{i+1}|)^{p-j} \right) \\
\end{align}

Thus, we get
\begin{align*}
\Exp_S \Exp_{x \sim \unif([0,1])}[|\hat{f}(x)-f^*(x)|^p ]& \leq  \Exp_S \left[ \frac{T_1 + T_2 +T_3}{n} \right] \\
\end{align*}
Since for any fixed $p$, the $p$-th moment of folded Gaussian is finite,
 \begin{align}
     \lim_{n\rightarrow \infty}  \frac{\Exp_S \left[T_1\right]}{n}= \lim_{n\rightarrow \infty}  \frac{\Exp_S \left[\left(2G/n+2|\eps_0|+|\eps_1|\right)^p\right]}{n} = 0. \label{eq:gird-term1-limit}
 \end{align}
 For the same reason,
 \begin{align}
     \lim_{n\rightarrow \infty}  \frac{\Exp_S \left[T_3\right]}{n}= \lim_{n\rightarrow \infty}  \frac{\Exp_S \left[\left(2G/n+|\eps_{n-1}|+|\eps_{n}|\right)^p\right]}{n} = 0 ~.\label{eq:gird-term3-limit}
 \end{align}
 Now,
 \begin{align*}
 \frac{\Exp_S \left[ T_2\right]}{n} &= \frac{1}{n} \cdot  \Exp_S \sum_{i=2}^{n-1} \left( \frac{2G}{n}+2|\eps_i|+2|\eps_{i-1}|+|\eps_{i-2}|+|\eps_{i+1}| \right)^p \\
 &= \frac{2^p}{n} \cdot  \Exp_S \sum_{i=2}^{n-1} \left( \frac{G}{n}+|\eps_i|+|\eps_{i-1}|+|\eps_{i-2}|+|\eps_{i+1}| \right)^p \\
     &\leq \frac{2^p}{n} \sum_{i=2}^{n-1} \Exp_{S} \left( (|\eps_i|+|\eps_{i-1}|+|\eps_{i-2}|+|\eps_{i+1}|)^p + \sum_{j=1}^{p} \binom{p}{j} \left(\frac{G}{n}\right)^j (|\eps_i|+|\eps_{i-1}|+|\eps_{i-2}|+|\eps_{i+1}|)^{p-j} \right) 
\end{align*}
Let $Y=|Y_1|+|Y_2|+|Y_3|+|Y_4|$, where $Y_i \iid \normal(0,\sigma^2)$, i.e. $Y$ is the sum of the absolute values of four independent Gaussians. Clearly, for any finite $p'$, we have that for some finite constant $B:=B(p')$
\[
\Exp[Y^{p'}]=B(p') \leq 4^{p'} \Exp |Y_1|^{p'} = 4^{p'} \cdot \sigma^{p'} \sqrt{\frac{2^{p'}}{\pi}}\Gamma \left( \frac{p'+1}{2}\right)~.
\]
Hence,
 \begin{align*}
     \frac{\Exp_S \left[ T_2\right]}{n} 
     &\leq \frac{2^p}{n} \sum_{i=2}^{n-1} \Exp_{S} \left( (|\eps_i|+|\eps_{i-1}|+|\eps_{i-2}|+|\eps_{i+1}|)^p + \sum_{j=1}^{p} \binom{p}{j} \left(\frac{G}{n}\right)^j (|\eps_i|+|\eps_{i-1}|+|\eps_{i-2}|+|\eps_{i+1}|)^{p-j} \right) \\
&\leq \frac{2^p}{n} \left( \sum_{i=2}^{n-1} \left( B(p)+ \sum_{j=1}^{p} \binom{p}{j} \left(\frac{G}{n}\right)^j B(p-j) \right)\right)\\
&= \frac{2^p(n-2)}{n}  \left( B(p)+ \sum_{j=1}^{p} \binom{p}{j} \left(\frac{G}{n}\right)^j B(p-j) \right)\\
\lim_{n\rightarrow \infty} \frac{\Exp_S \left[ T_2\right]}{n} 
& \leq \lim_{n \rightarrow \infty} \frac{2^p(n-2)}{n}  \left( B(p)+ \sum_{j=1}^{p} \binom{p}{j} \left(\frac{G}{n}\right)^j B(p-j) \right)\\
&= 2^p \cdot B(p) \leq 8^p \cdot \sigma^p \cdot \sqrt{\frac{2^p}{\pi}} \Gamma \left( \frac{p+1}{2}\right)~. \label{eq:grid-term2-limit}
 \end{align*}
Therefore, finally, we can analyze
 \begin{align*}
 \Exp_S \sup_{\hat{f} \in \ridgeless(S)} [L_p(\hat{f})] & = \Exp_S \left[ \Exp_{(x,y)\sim \dist} \left[ |\hat{f}(x)-y|^p\right] \right]\\
 & \leq \Exp_S \left[ \Exp_{x\sim \unif([0,1]),\eps\sim \normal(0,\sigma^2)} \left[ |\hat{f}(x)-f^*(x)+\eps|^p\right] \right]\\
 & \leq  2^p \left[ \Exp_S \Exp_{x\sim \unif([0,1]),\eps\sim \normal(0,\sigma^2)} \left[ |\hat{f}(x)-f^*(x)|^p+|\eps|^p\right] \right]\\
 & \leq 2^p  \left[ \Exp_S \Exp_{x\sim \unif([0,1])} \left[ |\hat{f}(x)-f^*(x)|^p \right]+ \Exp_{\eps\sim \normal(0,\sigma^2)} |\eps|^p \right]~.
 \end{align*}
 Taking the limit on both sides as $n$ tends to $\infty$,
 \begin{align*}
  \lim_{n\rightarrow \infty} \Exp_S \sup_{\hat{f} \in \ridgeless(S)} [L_p(\hat{f})] &\leq 2^p \lim_{n \rightarrow \infty} \left[ \Exp_S \Exp_{x\sim \unif([0,1])} \left[ |\hat{f}(x)-f^*(x)|^p \right]+ \Exp_{\eps\sim \normal(0,\sigma^2)} |\eps|^p \right]\\
  & =  2^p \left[ \lim_{n \rightarrow \infty} \Exp_S \left[ \frac{T_1+T_2+T_3}{n} \right]+ \sigma^p \cdot \sqrt{\frac{2^p}{\pi}} \Gamma \left( \frac{p+1}{2}\right) \right]\\
  &\leq 2^p \left(0+ 8^p \sigma^p \cdot \sqrt{\frac{2^p}{\pi}} \Gamma \left( \frac{p+1}{2}\right) +0+\sigma^p \cdot \sqrt{\frac{2^p}{\pi}} \Gamma \left( \frac{p+1}{2}\right) \right)\\
  &\leq \frac{18^p \sqrt{2^p} \cdot \sigma^p}{\sqrt{\pi}} \Gamma \left( \frac{p+1}{2}\right)
 \end{align*}
\begin{align*}
L_p^*=L_p(f^*)&=\Exp_{(x,y)\sim \dist} \left[ |f^*(x)-y|^p\right]\\
    & = \Exp_{\eps\sim \normal (0,\sigma^2) }\left[ |f^*(x)-f^*(x)+\eps|^p \right] = \Exp_{\eps\sim \normal (0,\sigma^2) }\left[ |\eps|^p \right] \\
    &=  \sigma^p\cdot \sqrt{\frac{2^p}{\pi}} \Gamma \left( \frac{p+1}{2}\right)
   % &=  \frac{\sigma \sqrt{2}}{\pi^{\frac{1}{2p}}} \Gamma \left( \frac{p+1}{2}\right)^{1/p} 
\end{align*}
Therefore, combining the two
$$\lim_{n\rightarrow \infty} \Exp_S \sup_{\hat{f} \in \ridgeless(S)} [L_p(\hat{f})] \leq 18^p L_p^*.$$
\end{proof}

==> l1_worst-case.tex <==
\section{Tempered Overfiiting with respect to $\ell_1$-loss}
 \begin{theorem} 
 For the joint distribution $\dist$, we have that
 \[
 \lim_{n \rightarrow \infty} \Exp_S \sup_{\hat{f} \in \ridgeless(S)} [L_1(\hat{f})] \leq 50 \, L_1^*~,
 \]
 where $L_1^*=L_1(f^*)$ is $\ell_1$ the Bayes risk for the distribution $\dist$.
 \end{theorem}
 \begin{proof}
Again, we will have $n$ inteervals of length $\ell_1,\dots,\ell_n$ such that $\sum_{i=1}^{n} \ell_i=1$. For any $i\in \{2,\dots,n-1\}$ and any $x\in [x_{i-1},x_i)$, by Lemma \ref{?},
 \[
 |\hat{f}(x)-f^*(x)| \leq \max\left\{ |g_i(x)-f^*(x)|, \min\{|g_{i+1}(x)-f^*(x)|, |g_{i-1}(x)-f^*(x)|\}\right\}
 \]
 \begin{align*}
      |\hat{f}(x)-f^*(x)| &\leq \max\left\{ |g_i(x)-f^*(x)|, \min\{|g_{i+1}(x)-f^*(x)|, |g_{i-1}(x)-f^*(x)|\}\right\}\\
      & \leq |g_i(x)-f^*(x)|+ \min\{|g_{i+1}(x)-f^*(x)|  , |g_{i-1}(x)-f^*(x)|\} \\
      \int_{x_{i-1}}^{x_i} |\hat{f}(x)-f^*(x)| \, dx \, & \leq   \int_{x_{i-1}}^{x_i} |g_i(x)-f^*(x)| \, dx + \int_{x_{i-1}}^{x_i} \min\{|g_{i+1}(x)-f^*(x)|  , |g_{i-1}(x)-f^*(x)|\} \, dx \\
      \sum_{i=2}^{n-1}\int_{x_{i-1}}^{x_i} |\hat{f}(x)-f^*(x)| \, dx \, & \leq  \sum_{i=2}^{n-1} \int_{x_{i-1}}^{x_i} |g_i(x)-f^*(x)| \, dx + \sum_{i=2}^{n-1}\int_{x_{i-1}}^{x_i} \min\{|g_{i+1}(x)-f^*(x)|  , |g_{i-1}(x)-f^*(x)|\} \, dx \\
 \end{align*}
Moreover, for $i \in \{1,n\}$
 \[
 |\hat{f}(x)-f^*(x)| \leq |g_i(x)-f^*(x)|
 \]
 Therefore,
 $$ \int_{x_{i-1}}^{x_i}  |\hat{f}(x)-f^*(x)| \, dx \, \leq \int_{x_{i-1}}^{x_i} |g_i(x)-f^*(x)| \, dx$$
 Combining the above:
 \begin{align*}
     \Exp_{x \sim \unif([0,1])} [|\hat{f}(x)-f^*(x)|] &= \int_{0}^{1} |\hat{f}(x)-f^*(x)| \, dx \\
     &= \sum_{i=1}^{n} \int_{x_{i-1}}^{x_i} |\hat{f}(x)-f^*(x)| \, dx \\
     & \leq \sum_{i=1}^{n} \int_{x_{i-1}}^{x_i} |g_i(x)-f^*(x)| \, dx \\
     & \hspace{2mm} + \sum_{i=2}^{n-1}\int_{x_{i-1}}^{x_i} \min\{|g_{i+1}(x)-f^*(x)|  , |g_{i-1}(x)-f^*(x)|\} \, dx 
 \end{align*}
 Therefore, taking expectation with respect to $S$ and considering the limit as $n$ approaches $\infty$:
 \begin{align*}
    \lim_{n \rightarrow \infty} \Exp_S  \sup_{\hat{f} \in \ridgeless (S)} [L_1(\hat{f})] & \leq \lim_{n \rightarrow \infty} \Exp_S \sum_{i=1}^{n} \int_{x_{i-1}}^{x_i} |g_i(x)-f^*(x)| \, dx \\
     & \hspace{2mm} + \lim_{n \rightarrow \infty} \Exp_S \sum_{i=2}^{n-1}\int_{x_{i-1}}^{x_i} \min\{|g_{i+1}(x)-f^*(x)|  , |g_{i-1}(x)-f^*(x)|\} \, dx\\
     & \leq \lim_{n \rightarrow \infty}  \Exp_S \left[ \Exp_{x\sim \unif([0,1])} \left[ |\hat{f}_{\text{spline}}-f^*(x)| \right] \right] \\
     & \hspace{2mm} + \underbrace{\lim_{n \rightarrow \infty} \Exp_S \sum_{i=2}^{n-1}\int_{x_{i-1}}^{x_i} \min\{|g_{i+1}(x)-f^*(x)|  , |g_{i-1}(x)-f^*(x)|\} \, dx }_{:=T}\\
    & \leq  2 \cdot 4^{p} \cdot \sigma^p \cdot\sqrt{\frac{2^{p}}{\pi}} \Gamma\left( \frac{p+1}{2}\right) + T\\
 \end{align*}
 Therefore, it basically boils down to analyzing
 $$T=\lim_{n \rightarrow \infty} \Exp_S \sum_{i=2}^{n-1}\int_{x_{i-1}}^{x_i} \min\{|g_{i+1}(x)-f^*(x)|  , |g_{i-1}(x)-f^*(x)|\} \, dx$$
 \end{proof}
 

==> linear_splines.tex <==
\section{Linear Splines}
We will sample $n-1$ points i.i.d. from $\dist$. For simplicity of exposition, we also assume that we get noisy labels corresponding to $x_0=0$ and $x_n=1$. We number the datapoints $S=\{(x_i,y_i): i=0,1,\dots,n\}$ such that
\begin{equation}
   0=x_0 \leq x_1 \leq x_2 \leq \dots \leq x_{n-1} \leq x_n=1, 
\end{equation}
\begin{equation}\label{eq:non-grid-dataset}
   \forall i \in [n], \hspace{1mm} y_i=f^*(x_i)+\eps_i\,\hspace{2mm} \text{where } \eps_i \sim \normal(0,\sigma^2).   
\end{equation}
Our goal is to analyze the risk of linear splines of the dataset $S$.
\begin{theorem}
 For the joint distribution specified as in the above, and any fixed $p \in \IN_{+}$, we have
 \[
 \lim_{n \rightarrow \infty} \Exp_S  [L_p(\hat{f}_{\text{spline}})] \leq c_p \, L_p^*~,
 \]
 where $L_p^*=L_p(f^*)$ is the Bayes error and $c_p$ is a constant that only depends on $p$.
\end{theorem}
\begin{proof}
 We have $n$ intervals in total: the $i$-th interval is $[x_{i-1},x_i)$. We denote their lengths by $\ell_1,\dots,\ell_n$ from left to right.
$$ \ell_i:= x_i-x_{i-1}.$$
Moreover, let $g_i:\IR \rightarrow \IR$ be the affine function joining the points $(x_{i-1},y_{i-1})$ and $(x_i,y_i)$. Thus, $g_i$ is the straight line joining the endpoints of the $i$-th interval. Then, 
%by definition 
the linear spline $\hat{f}_{\text{spline}}: [0,1]\rightarrow \IR$ satisfies
$$ \hat{f}_{\text{spline}}(x)= \sum_{i=1}^{n} g_i(x)\cdot \mathbf{1}\{x\in [x_{i-1},x_i)\}.$$
Fix any $i\in[n]$, and for any $x\in [x_{i-1},x_i)$,
\begin{align*}
 |\hat{f}_{\text{spline}}(x)-f^*(x)| &= |g_i(x)-f^*(x)| \\
 =&\left| y_{i-1}+ \frac{(y_{i}-y_{i-1})}{x_{i}-x_{i-1}} (x-x_{i-1})-f^*(x)\right|\\
 =& \left| f^*(x_{i-1})+\eps_{i-1} + \left(\frac{f^*(x_i)+\eps_i-f^*(x_{i-1})-\eps_{i-1}}{x_{i}-x_{i-1}}\right)(x-x_{i-1}) -f^*(x)\right| \\
 \leq & \left| f^*(x_{i-1}) -f^*(x)\right|+ |\eps_{i-1}|+ \left| \frac{G(x_i-x_{i-1})+\eps_i-\eps_{i-1}}{x_i-x_{i-1}} \right|  (x-x_{i-1})  \\
 \leq &  G(x-x_{i-1}) + |\eps_{i-1}|+ \left( \frac{G(x_i-x_{i-1})+|\eps_i|+|\eps_{i-1}|}{x_i-x_{i-1}} \right)  (x-x_{i-1})  \\
 \leq & G \cdot \ell_i + |\eps_{i-1}|+ \left( \frac{G \cdot \ell_i +|\eps_i|+|\eps_{i-1}|}{\ell_i} \right) \cdot \ell_i\\
 = & 2G \cdot \ell_i + |\eps_i|+2 |\eps_{i-1}|.
\end{align*}

Hence,
\begin{align}
  \Exp_{x \sim \unif{[0,1]}} \left[ |\hat{f}_{\text{spline}}(x)-f^*(x)|^p \right] &\leq \sum_{i=1}^{n} \prob{x\in [x_{i-1},x_i)} \Exp \left[|\hat{f}_{\text{spline}}(x)-f^*(x)|^p \mid x\in [x_{i-1},x_i) \right]  \nonumber\\
  & \leq \sum_{i=1}^{n} \ell_i \left( 2G \cdot \ell_i + |\eps_i|+2 |\eps_{i-1}|\right)^p \nonumber\\
  &= \sum_{i=1}^{n} \left[ \ell_i \left( (|\eps_i|+2|\eps_{i-1}|)^p +\sum_{j=1}^{p} \binom{p}{j} (2G \cdot \ell_i)^j (|\eps_i|+2|\eps_{i-1}|)^{p-j} \right) \right]
\end{align}
Therefore, taking the expectation with respect to $S$,
\begin{align*}
    \Exp_S \left[  \Exp_{x \sim \unif{[0,1]}} \left[ |\hat{f}_{\text{spline}}(x)-f^*(x)|^p \right] \right] & \leq \sum_{i=1}^{n} \Exp_S \left[ \ell_i \left( (|\eps_i|+2|\eps_{i-1}|)^p +\sum_{j=1}^{p} \binom{p}{j} (2G \cdot \ell_i)^j (|\eps_i|+2|\eps_{i-1}|)^{p-j} \right) \right]\\
    & \leq  \sum_{i=1}^{n}\left( \Exp_S \left[ \ell_i(|\eps_i|+2|\eps_{i-1}|)^p \right] +\sum_{j=1}^{p} \binom{p}{j} (2G)^j \cdot \Exp_S \left[ (\ell_i)^{j+1} (|\eps_i|+2|\eps_{i-1}|)^{p-j} \right] \right) \\
    &= \sum_{i=1}^{n} \sum_{j=1}^{p} \Exp_S \left[ T_j\right],
\end{align*}
where  $T_j:=\binom{p}{j}(2G)^j {\ell_i}^{j+1} (|\eps_i|+2|\eps_{i-1}|)^{p-j}$. Let $Y_1,Y_2 \iid \normal(0,\sigma^2)$. And let $Y=2|Y_1|+|Y_2|$. Then it is well-known that, for any finite $p'$, $\Exp[Y^{p'}]$ is finite, which we denote by $B(p')$.
\begin{align*}
    B(p')&=\Exp \left[ Y^{p'} \right] = \Exp \left[(2|Y_1|+|Y_2|)^{p'} \right] \leq 2^p \Exp \left[(|Y_1|+|Y_2|)^{p'} \right]\\
    & \leq 4^{p'} \Exp \left[ |Y_1|^{p'}+|Y_2|^{p'} \right] \leq 2 \cdot 4^{p'} \cdot \sigma^{p'} \cdot \sqrt{\frac{2^{p'}}{\pi}} \Gamma\left( \frac{p'+1}{2}\right).
\end{align*}
Also, we now need to characterize the distribution of the interval spacings $(\ell_1,\dots,\ell_n)$ and calculate the moments of each $\ell_i$. Let 
%$X_1,\dots,X_n \iid \text{Exponential}(1)$ 
$X_1,\dots,X_n \iid \text{Exp}(1)$ 
and $X=\sum_{i=1}^{n} X_i$. It is well-known that \nirmit{cite}
$$(\ell_1,\dots,\ell_n) \sim \left( \frac{X_1}{X},\dots, \frac{X_n}{X}\right).$$
Thus, the $\ell_i$'s are identically distributed. For any fixed $q$, calculating the $q$-th moment of $\ell_i$ for any $i\in[n]$
\begin{align*}
    \Exp [\ell_i^q] & =\Exp[\ell_1^q] = \Exp \left[ \frac{X_1^q}{(X_1+\dots+X_n)^q}\right] \leq \Exp \left[ \frac{X_1^q}{(X_2+\dots+X_n)^q}\right] \leq \Exp[X_1^q] \Exp \left[ \frac{1}{(X_2+\dots+X_n)^q}\right]~. 
\end{align*}
Letting $Z=X_2+\dots+X_n$, we have $Z\sim \Gamma(n-1,1)$. Therefore,
\begin{align*}
    \Exp \left[ \frac{1}{Z^q}\right] &= \int_{0}^{\infty} \frac{1}{z^q} \cdot \frac{z^{n-2}e^{-z}}{\Gamma(n-1)} dz\\
    &= \frac{1}{\Gamma(n-1)}\int_{0}^{\infty}  z^{n-q-2}e^{-z} dz\\
    &= \frac{\Gamma(n-q-1)}{\Gamma(n-1)}=\Theta \left( \frac{1}{n^q}\right)~.
\end{align*}
Therefore, using the fact that $\Exp[X_1^q]=q!$, we get
\begin{align*}
    \Exp [\ell_i^q] & \leq  \Exp \left[ X_1^q \right]  \cdot \Exp \left[ \frac{1}{(X_2+\dots+X_n)^q}\right] = \frac{q!}{\Theta(n^q)}.
\end{align*}
Combining this we can find the expectation of $T_j$
\begin{align*}
  \Exp_S \left[ T_j \right]&= \binom{p}{j} (2G)^{j} \cdot \Exp_S \left[ (\ell_i)^{j+1} (|\eps_i|+2|\eps_{i-1}|)^{p-j} \right]\\
&= \binom{p}{j} (2G)^{j} \cdot \Exp[ (\ell_i)^{j+1} ] \Exp[ (|\eps_i|+2|\eps_{i-1}|)^{p-j} ]  \\
&= \Theta\left(\frac{1}{n^{j+1}} \right)~. 
\end{align*}
Finally, combining substituting this in the above:
\begin{align*}
    \Exp_S \left[  \Exp_{x \sim \unif{[0,1]}} \left[ |\hat{f}_{\text{spline}}(x)-f^*(x)|^p \right] \right] 
    & \leq  \sum_{i=1}^{n}\left( \Exp \left[ \ell_i(|\eps_i|+2|\eps_{i-1}|)^p \right] +\sum_{j=1}^{p} \binom{p}{j} (2G)^j \cdot \Exp \left[ (\ell_i)^{j+1} (|\eps_i|+2|\eps_{i-1}|)^{p-j} \right] \right) \\
    & = \sum_{i=1}^{n} \left[ \frac{B(p)}{n} + \sum_{j=1}^{p} \Theta\left( \frac{1}{n^{j+1}}\right)\right] \\
    & =  B(p) + \sum_{j=1}^{p} \Theta\left( \frac{1}{n^{j}}\right).
\end{align*}
Taking the limit as $n$ approaches infinity, we get:
$$ \lim_{n \rightarrow \infty} \Exp_S \left[  \Exp_{x \sim \unif{[0,1]}} \left[ |\hat{f}_{\text{spline}}(x)-f^*(x)|^p \right] \right] \leq B(p) \leq 2 \cdot 4^{p} \cdot \sigma^p \cdot\sqrt{\frac{2^{p}}{\pi}} \Gamma\left( \frac{p+1}{2}\right).$$
Therefore, finally, we can analyze
 \begin{align*}
 \Exp_S L_p(\hat{f}_{\text{spline}}) & = \Exp_S \left[ \Exp_{(x,y)\sim \dist} \left[ |\hat{f}_{\text{spline}}(x)-y|^p\right] \right]\\
 & \leq \Exp_S \left[ \Exp_{x\sim \unif([0,1]),\eps\sim \normal(0,\sigma^2)} \left[ |\hat{f}_{\text{spline}}(x)-f^*(x)+\eps|^p\right] \right]\\
 & \leq  2^p \cdot  \Exp_S \Exp_{x\sim \unif([0,1]),\eps\sim \normal(0,\sigma^2)} \left[ |\hat{f}(x)-f^*(x)|^p+|\eps|^p\right]\\
 & \leq  2^p \left[ \Exp_S \Exp_{x\sim \unif([0,1])} \left[ |\hat{f}(x)-f^*(x)|^p \right]+ \Exp_{\eps\sim \normal(0,\sigma^2)} |\eps|^p \right]
 \end{align*}
 Taking the limit on both sides as $n$ tends to $\infty$,
 \begin{align*}
  \lim_{n\rightarrow \infty} \Exp_S L_p(\hat{f}_0)  &\leq 2^p \cdot \lim_{n \rightarrow \infty} \left[ \Exp_S \Exp_{x\sim \unif([0,1])} \left[ |\hat{f}(x)-f^*(x)|^p \right]+ \Exp_{\eps\sim \normal(0,\sigma^2)} |\eps|^p \right]\\
  & \leq  2^p \left[ 2 \cdot 4^{p} \cdot \sigma^p \cdot\sqrt{\frac{2^{p}}{\pi}} \Gamma\left( \frac{p+1}{2}\right) + \sigma^p \cdot \sqrt{\frac{2^p}{\pi}} \Gamma \left( \frac{p+1}{2}\right) \right]\\
  & = (2\cdot 8^p + 2^p) \cdot \sigma^p \cdot \sqrt{\frac{2^p}{\pi}} \Gamma \left( \frac{p+1}{2}\right)\\
  &= c_p L_p^*.
 \end{align*}
 \end{proof}
